Sensitivity Analysis in Population Shares

Empirical work often relies on assumptions on the distribution of random variables, such as potential outcomes or latent variables, to identify some parameter of interest. We introduce a unified framework for assessing the sensitivity of a target estimand to relaxing these distributional assumptions for a given share of the population. We derive bounds on the values the estimand can take as this share varies between 0 and 1, and compute the bounds using tractable finite-dimensional programs. We propose plug-in estimators for the bounds and characterize their large sample properties. We also show that our bounds recover exact nonparametric sharp bounds at no additional computational cost, and introduce summary measures that separate misspecification uncertainty from sampling uncertainty and rank studies by their robustness. We apply our framework to assess the robustness of (i) average treatment effects in randomized experiments with attrition, (ii) counterfactual predictions in structural models, and (iii) formula instruments. We provide R and Python packages implementing all our methods.

==> preamble-SA.tex <==
\PassOptionsToPackage{nopatch=footnote}{microtype}
\usepackage{natbib}
\newcommand{\citetapos}[1]{\citeauthor{#1}'s \citeyearpar{#1}}
\usepackage[nottoc,notbib]{tocbibind}
\usepackage[dvipsnames,usenames]{color}
\usepackage[table]{xcolor}

\usepackage{adjustbox, algorithm, algpseudocode, amsfonts, amsmath, amssymb, amsthm, appendix, array, authblk, bigstrut, bm, bbm, booktabs, caption, commath, datetime, dsfont, enumerate, enumitem, environ, epigraph, epsfig, eurosym, graphicx, latexsym, longtable, mathtools, mathrsfs, microtype, morefloats, multirow, pifont, pdflscape, rotating, siunitx, subcaption, tikz, threeparttable, ulem, verbatim}
\usepackage{accents}   % \accentset for \rhopad, \underaccent for \ubar; load after amsmath
\usepackage{hyperref}

\usepackage[singlespacing]{setspace}
\usepackage[right=1.75cm, left=1.75cm, top=1.75cm, bottom=1.75cm]{geometry} % 2cm before the 2026-09-18 page-budget pass
\usepackage[font={bf},justification=centering]{caption}
\usepackage[referable]{threeparttablex}
\usepackage[section]{placeins}
\usepackage[hang,flushmargin]{footmisc}
\usepackage{titlesec}
\titlespacing*{\section}{0pt}{2ex}{1ex}
\titlespacing*{\subsection}{0pt}{1.5ex}{0.8ex}
\titlespacing*{\subsubsection}{0pt}{1.2ex}{0.6ex}

\makeatletter
\let\lnk@makefntext\@makefntext
\long\def\@makefntext#1{\lnk@fntarget\lnk@makefntext{#1}}
\def\lnk@fntarget{%
  \ifx\Hy@footnote@currentHref\@empty\else
    \ifx\Hy@footnote@currentHref\lnk@lastfn\else
      \global\let\lnk@lastfn\Hy@footnote@currentHref
      \Hy@raisedlink{\hyper@anchorstart{\Hy@footnote@currentHref}\hyper@anchorend}%
    \fi
  \fi}
\let\lnk@lastfn\@empty
\let\lnk@deferred@thm@head\deferred@thm@head
\def\deferred@thm@head#1{%
  \ifx\@empty\dth@counter
    \lnk@deferred@thm@head{#1}%
  \else
    \lnk@deferred@thm@head{%
      \Hy@raisedlink{\hyper@anchorstart{\Hy@dth@currentHref}\hyper@anchorend}#1}%
    \let\dth@counter\@empty
  \fi}
\makeatother

\newcommand{\sym}[1]{#1}

\usdate
\newdateformat{monthyeardate}{%
	\monthname[\THEMONTH], \THEYEAR}

\newcommand{\harvardand}{and}
\newcounter{bean}
\newenvironment{alineas}{\begin{list}{\Alph{bean}.}{\usecounter{bean}}}{\end{list}}
\renewcommand{\figurename}{Fig.}


\newcommand{\fred}[1]{{ \textcolor{red}{ \bf [ \footnotesize #1 ]}}}


\newsavebox{\mybox}\newsavebox{\mysim}
\renewcommand{\qedsymbol}{$\blacksquare$}                      % end of proof black square

\theoremstyle{plain}
\newtheorem{defi}{Definition}         % own counter (defi)
\newtheorem{thm}{Theorem}             % shared "results" counter (Theorem/Proposition/Lemma/...)
\newtheorem{prop}[thm]{Proposition}   % shares the results counter
\newtheorem{ax}{Axiom}                % own counter (ax)
\newtheorem{cor}[thm]{Corollary}      % shares the results counter
\newtheorem{assump}{Assumption}       % own counter
\newtheorem{lemma}[thm]{Lemma}        % shares the results counter
\theoremstyle{definition}             % theorems below not in italic
\newtheorem{rem}{Remark}              % own counter
\newtheorem{ex}{Example}              % own counter
\newtheorem*{prf}{Proof}
\makeatletter
\newcommand{\@endmark}[1]{%
  \unskip\nobreak\hfil\penalty50\hskip1em\hbox{}\nobreak\hfil#1%
  \parfillskip=\z@\finalhyphendemerits=\z@\relax}
\renewcommand{\endrem}{\@endmark{\ding{168}}\endtrivlist\@endpefalse}
\renewcommand{\endex}{\@endmark{\ding{169}}\endtrivlist\@endpefalse}
\makeatother
\renewcommand\theassump{\arabic{assump}}         % Arabic numbering for assumptions
\renewcommand{\thesubfigure}{\roman{subfigure}}  % Roman numbering for subfigures

\input{notation.tex}


\input{figures/legend_macros.tex}


\definecolor{ptonorange}{RGB}{232,119,34}
\hypersetup{colorlinks=true,linkcolor=ptonorange,filecolor=ptonorange,urlcolor=ptonorange,citecolor=ptonorange}
\colorlet{DarkRed}{red!70!black}
\definecolor{DarkBlue}{rgb}{0,0,0.9}
\colorlet{DarkGreen}{green!70!black}
\definecolor{tvblue}{HTML}{1F4E79}   % TV neighborhood in Fig. (minimal example); matches the R figure palette
\definecolor{answ}{RGB}{0, 0, 139}

\allowdisplaybreaks                 % Allow multiple-page equations


\usepackage{algorithm}
\usepackage{algpseudocode}
\newcommand\Algphase[1]{%
\vspace*{-.2\baselineskip}\Statex\hspace*{\dimexpr-\algorithmicindent--4pt\relax}\rule{\textwidth}{0.4pt}%
\Statex\hspace*{\dimexpr-\algorithmicindent--5pt\relax}\textbf{#1}%
\vspace*{-.7\baselineskip}\Statex\hspace*{\dimexpr-\algorithmicindent--4pt\relax}\rule{\textwidth}{0.4pt}%
}

\newcounter{algsubstate}
\renewcommand{\thealgsubstate}{\alph{algsubstate}}
\newenvironment{algsubstates}
  {\setcounter{algsubstate}{0}%
   \renewcommand{\State}{%
     \stepcounter{algsubstate}%
     \Statex\hspace*{\dimexpr-\algorithmicindent--24pt\relax} {\footnotesize\thealgsubstate:}\space}}
  {}


\usepackage{tikz, pgfplots}
\pgfplotsset{compat=1.18}
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{
arrows.meta,
automata,
backgrounds,
bending,
calc,
decorations.pathreplacing,
shapes, 
shapes.geometric,
shapes.misc,
shapes.multipart,
positioning}

\usepackage{etoolbox}

\makeatletter

\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}

\patchcmd{\NAT@citex}
  {\@citea\NAT@hyper@{%
     \NAT@nmfmt{\NAT@nm}%
     \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
       {\@citeb\@extra@b@citeb}%
     \NAT@date}}
  {\@citea\NAT@nmfmt{\NAT@nm}%
   \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
  {}{}

\theoremstyle{plain}                    % restore italic body for Theorem
\newtheorem{theorem}[thm]{Theorem}      % shares the results counter (thm)
\theoremstyle{definition}               % algo/remark stay upright
\newtheorem{algo}{Algorithm}            % own counter
\newtheorem*{remark}{Remark}            % unnumbered, matches source

\renewcommand{\thesection}{SA\arabic{section}}
\usepackage{tocloft}
\makeatletter
\renewcommand{\numberline}[1]{%
  \@cftbsnum #1\@cftasnum~\@cftasnumb%
}
\makeatother


\setcounter{figure}{0}
\renewcommand\thefigure{SA-\arabic{figure}} 
\setcounter{table}{0}
\renewcommand{\thetable}{SA-\arabic{table}}
\setcounter{algorithm}{0}
\renewcommand{\thealgorithm}{SA-\arabic{algorithm}}
\renewcommand{\thethm}{SA-\arabic{thm}}     % Theorem/Proposition/Lemma/Corollary (shared)
\renewcommand{\thedefi}{SA-\arabic{defi}}   % Definition (own counter)
\renewcommand{\theax}{SA-\arabic{ax}}       % Axiom (own counter)
\renewcommand{\theex}{SA-\arabic{ex}}       % Example (own counter)
\renewcommand{\therem}{SA-\arabic{rem}}     % Remark (own counter)
\renewcommand{\thealgo}{SA-\arabic{algo}}   % Algorithm (own counter)
\renewcommand{\theassump}{SA-\arabic{assump}}

\renewcommand{\topfraction}{0.9}        % up to 90% of a page may be a top float
\renewcommand{\bottomfraction}{0.8}     % up to 80% may be a bottom float
\renewcommand{\textfraction}{0.08}      % require only 8% of a text page be text
\renewcommand{\floatpagefraction}{0.75} % a float page must be >=75% full
\setcounter{topnumber}{3}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{5}

\renewcommand{\refname}{Supplement References}

\setcounter{tocdepth}{2}

